Aligning Books and Movies: Towards Story-like Visual Explanations by Watching Movies and Reading Books

Books are a rich source of both fine-grained information, how a character, an object or a scene looks like, as well as high-level semantics, what someone is thinking, feeling and how these states evolve through a story. This paper aims to align books to their movie releases in order to provide rich descriptive explanations for visual content that go semantically far beyond the captions available in current datasets. To align movies and books we exploit a neural sentence embedding that is trained in an unsupervised way from a large corpus of books, as well as a video-text neural embedding for computing similarities between movie clips and sentences in the book. We propose a context-aware CNN to combine information from multiple sources. We demonstrate good quantitative performance for movie/book alignment and show several qualitative examples that showcase the diversity of tasks our model can be used for.

==> retrieval.tex <==
\begin{table}[t!]
\tiny
\vspace{-3mm}
\hspace{-2mm}\addtolength{\tabcolsep}{-3.4pt}
\begin{tabular}{|p{0.84cm}|p{0.006cm}p{0.72cm}p{0.006cm}p{0.72cm}p{0.006cm}p{0.72cm}p{0.006cm}p{0.72cm}p{0.006cm}p{0.72cm}p{0.006cm}p{0.72cm}p{0.006cm}p{0.84cm}|}
\hline
\includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_dvd.jpg} 
& \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg}  
& \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
& \rotatebox{90}{Green Mile}  & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
& \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
& \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg}
& \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg}
& \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg}\\
%American Psycho & American Psycho & One Flew  &  Green Mile &  Harry Potter &   Shawshank Redemption&     Fight Club&     The Road &     The Firm &     Brokeback Mountain\\
& & 100	&  &23.1	& &20.31	& &16.67	& &15.02	& &13.53	& &10.55\\
\hline
\includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_dvd.jpg}
& \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg}
& \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg} 
& \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
& \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg}  
& \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg}
& \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg}
& \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg}\\
%Harry Potter &     Harry Potter  & American Psycho &     One Flew &    Green Mile &     Shawshank Redemption&     Fight Club&        The Firm &    Brokeback Mountain & The Road \\
& & 100 &	 &33.54 &&	21.07&&	19.72	&&15.2	&&12.91&&	12.33\\
\hline
\end{tabular}
\vspace{-3mm}
\caption{{\bf Book ``retrieval'' results}. For a {\bf movie} (left), we rank  books wrt to their alignment similarity with the movie.  }
\label{fig:retrieval}
\vspace{-3mm}
\end{table}

==> retrieval_full.tex <==
\begin{table*}[h]\tiny
\centering
\hspace{-2mm}\addtolength{\tabcolsep}{-2.2pt}
\begin{tabular}{|c|p{-0.0cm}cp{0.00cm}cp{0.00cm}cp{0.00cm}cp{0.00cm}cp{0.00cm}cp{0.00cm}cp{0.00cm}cp{0.00cm}c|}
\hline
\multicolumn{1}{|>{\columncolor{bgr}}c|}{} & \multicolumn{18}{>{\columncolor{gr}}c|}{}\\[-0.6mm]
\multicolumn{1}{|>{\columncolor{bgr}}c|}{\sc\small movie} & \multicolumn{18}{>{\columncolor{gr}}c|}{\sc\small books}\\[-0.6mm]
\multicolumn{1}{|>{\columncolor{bgr}}c|}{\tiny} & \multicolumn{18}{>{\columncolor{gr}}c|}{\tiny}\\
\hline
\includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_dvd.jpg}
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg}\\ 
Fight Club    & & 100.0 & & 27.4 & & 27.4 & & 26.1 & & 25.8 & & 25.7 & & 23.6 & & 23.1 & & 19.9\\ 
 \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_dvd.jpg}
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg}\\ 
 Green Mile   & & 100.0 & & 22.2 & & 20.8 & & 20.2 & & 20.1 & & 19.5 & & 19.4 & & 17.7 & & 16.2\\ 
  \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_dvd.jpg}
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
 & \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg}\\ 
 Harry Potter   & & 100.0 & & 23.7 & & 22.9 & & 22.8 & & 22.5 & & 22.4 & & 22.0 & & 21.3 & & 20.5\\ 
  \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_dvd.jpg} 
 & \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg}\\ 
 American Pyscho   & & 100.0 & & 50.2 & & 47.5 & & 47.4 & & 46.1 & & 44.2 & & 44.0 & & 43.8 & & 43.4\\ 
   \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/flew_dvd.jpg} 
 & \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg}\\ 
 One Flew Over...    & & 100.0 & & 75.2 & & 74.1 & & 71.8 & & 68.9 & & 68.0 & & 67.3 & & 64.1 & & 64.0\\ 
    \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_dvd.jpg}  
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg}\\ 
 Shawshank ...   & & 100.0 & & 48.5 & & 46.1 & & 41.7 & & 40.7 & & 39.6 & & 38.5 & & 36.5 & & 35.9\\ 
  \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_cover.jpg}   
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg}\\ 
 The Firm   & & 100.0 & & 57.2 & & 55.9 & & 55.6 & & 55.2 & & 51.0 & & 49.5 & & 48.1 & & 46.8\\ 
      \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokeback_dvd.jpg}  
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg}\\ 
 Brokeback ...    & & 100.0 & & 34.2 & & 33.2 & & 32.1 & & 32.1 & & 32.0 & & 30.5 & & 29.8 & & 28.6\\ 
      \includegraphics[width=0.074\textwidth, height=12mm]{figs/covers/theroad_dvd.jpg}  
 & \rotatebox{90}{The Road} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{One Flew Over...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{American Pyscho} & \includegraphics[width=0.05\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg}\\ 
 The Road    & & 100.0 & & 35.1 & & 34.9 & & 34.0 & & 33.0 & & 32.6 & & 31.6 & & 31.6 & & 31.6\\ 
\hline
\end{tabular}
\vspace{-0mm}
\caption{{\bf Book ``retrieval'' results}. For a {\bf movie} (left), we rank  books wrt to their alignment similarity with the movie.  We normalize the similarity to be 100 for the highest scoring book.}
\label{fig:retrieval}
\vspace{-0mm}
\end{table*}

==> retrieval_full1.tex <==
\begin{table}[t!]\tiny
\vspace{-2mm}
\centering
\hspace{-2mm}\addtolength{\tabcolsep}{-4.8pt}
\begin{tabular}{|c|p{1.1mm}cp{1.1mm}cp{1.1mm}cp{1.1mm}cp{1.1mm}cp{1.1mm}cp{1.1mm}c|}
\hline
\multicolumn{1}{|>{\columncolor{bgr}}c|}{} & \multicolumn{14}{>{\columncolor{gr}}c|}{}\\[-0.6mm]
\multicolumn{1}{|>{\columncolor{bgr}}c|}{\sc\small movie} & \multicolumn{14}{>{\columncolor{gr}}c|}{\sc\small books}\\[-0.6mm]
\multicolumn{1}{|>{\columncolor{bgr}}c|}{\tiny} & \multicolumn{14}{>{\columncolor{gr}}c|}{\tiny}\\
\hline
\includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/fightclub_dvd.jpg}
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{American Psy.} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{One Flew...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/brokebackmountain_book.jpg}\\ 
% & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
 %& \rotatebox{90}{Green Mile} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/greenmile_book.jpg}\\ 
Fight Club    & & 100.0 & & 27.4 & & 27.4 & & 26.1 & & 25.8 & & 25.7 & & 23.6\\% & & 23.1 & & 19.9\\ 
 \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/greenmile_dvd.jpg}
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{One Flew...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{American Psy.} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_book.jpg}\\ 
% & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
% & \rotatebox{90}{Fight Club} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/fightclub_book.jpg}\\ 
 Green Mile   & & 100.0 & & 22.2 & & 20.8 & & 20.2 & & 20.1 & & 19.5 & & 19.4\\% & & 17.7 & & 16.2\\ 
  \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/harrypotter_dvd.jpg}
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/harrypotter_book.jpg} 
 & \rotatebox{90}{American Psy.} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{One Flew...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_book.jpg} \\
% & \rotatebox{90}{Green Mile} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
% & \rotatebox{90}{Fight Club} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/fightclub_book.jpg}\\ 
 Harry Potter   & & 100.0 & & 23.7 & & 22.9 & & 22.8 & & 22.5 & & 22.4 & & 22.0\\% & & 21.3 & & 20.5\\ 
  \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/americanpsycho_dvd.jpg} 
 & \rotatebox{90}{American Psy.} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{One Flew...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/greenmile_book.jpg}\\ 
% & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
% & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg}\\ 
 American Psy.   & & 100.0 & & 50.2 & & 47.5 & & 47.4 & & 46.1 & & 44.2 & & 44.0\\% & & 43.8 & & 43.4\\ 
   \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/flew_dvd.jpg} 
 & \rotatebox{90}{One Flew...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/harrypotter_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{American Psy.} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/brokebackmountain_book.jpg} \\
% & \rotatebox{90}{Green Mile} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
 %& \rotatebox{90}{The Road} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/theroad_book.jpg}\\ 
 One Flew...    & & 100.0 & & 75.2 & & 74.1 & & 71.8 & & 68.9 & & 68.0 & & 67.3\\% & & 64.1 & & 64.0\\ 
    \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_dvd.jpg}  
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{One Flew...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{American Psy.} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/fightclub_book.jpg} \\
% & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg} 
 %& \rotatebox{90}{Green Mile} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/greenmile_book.jpg}\\ 
 Shawshank ...   & & 100.0 & & 48.5 & & 46.1 & & 41.7 & & 40.7 & & 39.6 & & 38.5\\% & & 36.5 & & 35.9\\ 
  \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_cover.jpg}   
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{American Psy.} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{One Flew...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/harrypotter_book.jpg} \\
% & \rotatebox{90}{Fight Club} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/fightclub_book.jpg} 
 %& \rotatebox{90}{The Road} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/theroad_book.jpg}\\ 
 The Firm   & & 100.0 & & 57.2 & & 55.9 & & 55.6 & & 55.2 & & 51.0 & & 49.5\\% & & 48.1 & & 46.8\\ 
      \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/brokeback_dvd.jpg}  
 & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/brokebackmountain_book.jpg} 
 & \rotatebox{90}{One Flew...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{American Psy.} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/americanpsycho_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{The Road} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_book.jpg}\\ 
% & \rotatebox{90}{Green Mile} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/greenmile_book.jpg} 
 %& \rotatebox{90}{Harry Potter} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/harrypotter_book.jpg}\\ 
 Brokeback ...    & & 100.0 & & 34.2 & & 33.2 & & 32.1 & & 32.1 & & 32.0 & & 30.5 \\%& & 29.8 & & 28.6\\ 
      \includegraphics[width=0.044\textwidth, height=10.4mm,trim=50 0 50 0,clip=true]{figs/covers/theroad_dvd.jpg}  
 & \rotatebox{90}{The Road} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/theroad_book.jpg} 
 & \rotatebox{90}{The Firm} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/thefirm_book.jpg} 
 & \rotatebox{90}{One Flew...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/cukoo_book1.jpg} 
 & \rotatebox{90}{Fight Club} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/fightclub_book.jpg} 
 & \rotatebox{90}{Green Mile} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/greenmile_book.jpg} 
 & \rotatebox{90}{Shawshank ...} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/shawshank_book.jpg} 
 & \rotatebox{90}{Harry Potter} & \includegraphics[width=0.044\textwidth, height=10.4mm]{figs/covers/harrypotter_book.jpg}\\ 
% & \rotatebox{90}{Brokeback ...} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/brokebackmountain_book.jpg} 
 %& \rotatebox{90}{American Pyscho} & \includegraphics[width=0.044\textwidth, height=12mm]{figs/covers/americanpsycho_book.jpg}\\ 
 The Road    & & 100.0 & & 35.1 & & 34.9 & & 34.0 & & 33.0 & & 32.6 & & 31.6\\% & & 31.6 & & 31.6\\ 
\hline
\end{tabular}
\vspace{-2mm}
\caption{{\bf Book ``retrieval''}. For a movie (left), we rank  books wrt to their alignment similarity with the movie.  We normalize similarity to be 100 for the highest scoring book.}
\label{fig:retrieval}
\vspace{-1mm}
\end{table}
